A Comparative Framework for Evaluating Foundation Models on Tabular Data: A Case Study in Healthcare

Tabular data is the most common format in clinical practice, encompassing laboratory results, medication records, diagnostic codes, and patient demographics. As foundation models for tabular data have grown in number and variety, a practical question has become harder to answer: which model should a clinician or data scientist actually choose for a given task, and why? Existing surveys catalogue what these models can do, but they stop short of providing a structured way to compare them against the specific demands of a real application. We introduce \system{}, a comparative evaluation framework that scores and ranks tabular foundation models (TFMs) across six clinically meaningful dimensions: how well a model generalizes to new datasets, how effectively it protects patient privacy, how much data it needs to perform well, how it scales with growing datasets and feature spaces, how interpretable its predictions are to clinicians, and how fairly it performs across patient subgroups. Each dimension is broken down into measurable sub-components, and groups of sub-components can optionally be combined into supplementary compound scores, called super-metrics, that provide a diagnostic view of how a model performs across several dimensions simultaneously. To show how the framework works in practice, we apply it to two healthcare use cases, screening for iron deficiency and predicting heart failure, demonstrating how the same set of metrics leads to different model rankings depending on what matters most in each clinical context. We also provide a taxonomy of 45 TFMs organized by their underlying architecture, which serves as a reference for researchers and practitioners looking to navigate this rapidly expanding field.

==> drafts/other.tex <==
privacy sub metrics

    
    Assesses the model’s vulnerability to membership inference attacks, where adversaries attempt to determine if specific data points were part of the training set. It is calculated as the probability that an attacker can correctly identify whether a sample was part of the training data. A lower probability indicates better privacy protection, more formally,

    \begin{LARGE}
    \begin{equation}
        MIR = 1 - \left[ \frac{\mathcal{P}(correct) - 0.5}{H(A) + \mathcal{P}(FP) + \mathcal{P}(FN)} \right]
    \end{equation}
    \end{LARGE}

    Where $\mathcal{P}(correct)$ indicates the probability that the attacker correctly infers membership and $\mathcal{P}(FP)$ shows the probability that the attacker incorrectly infers that a non-member is a member, while $\mathcal{P}(FN)$ counts for the probability that the attacker incorrectly infers that a member is not a member. Besides, $H()$ is the Entropy function, measuring uncertainty or randomness, and $A$ is the attacker’s confidence level or degree of belief in their inference. Here, MIR values close to 1 indicate strong resistance to inference attacks.





    
    
    
    
    \textbf{Differential Privacy Compliance (DPC):} Measures the degree to which the model adheres to differential privacy standards, which add noise to data or model outputs to protect individual information. It is assessed based on the differential privacy parameter $\epsilon$, which quantifies privacy loss. Lower values of $\epsilon$ signify stronger privacy guarantees, more formally:
    
    \begin{LARGE}
    \begin{equation}
        DPC = \frac{\mathcal{P} \times \left( \frac{1}{1 + e^\epsilon} \right)}{\mathcal{P} + \left( \frac{1}{1 + e^\epsilon} \right)}
    \end{equation}
    \end{LARGE}

    Values closer to 1 suggest high compliance with privacy standards.




    \textbf{Data Reconstruction Attack Resistance (DRAR):} Evaluates the model's ability to prevent attackers from reconstructing original data from model outputs or gradients. It is measured as the success rate of reconstruction attacks, with lower success rates indicating better resistance, more formally,

    \begin{LARGE}
    \begin{equation}
        DRAR = 1 - \mathcal{P}_{Successful\_Reconstruction}
    \end{equation}
    \end{LARGE}

    A higher value indicates better resistance to data reconstruction attacks.



    \textbf{Performance with Reduced Data (PRD):} Measures the model’s ability to maintain performance when trained on a subset of the available data. This evaluates the model’s learning efficiency with less data. It is assessed by comparing the performance (e.g., accuracy, F1 score) of the model trained on a reduced dataset versus the full dataset., more formally:

    \begin{LARGE}
    \begin{equation}
        PRD = \left( 1 + \frac{\mathcal{P}_{reduced} - \mathcal{P}_{full}}{\left( \frac{\mathcal{P}_{reduced} + \mathcal{P}_{full}}{2} \right)} \right) / 2
    \end{equation}
    \end{LARGE}
    
    Values close to 1 indicate strong improvements and the model performs well even with significantly less data while values close to 0 indicate strong declines. A value of 0.5 would indicate no change.


    \textbf{Few-Shot Learning Capability (FLC):} assesses the foundation model's ability to generalize from a minimal number of labeled examples per class, demonstrating its capacity to learn effectively from limited instances. This metric captures not only the model's performance in a few-shot scenario but also considers the complexity of the task, the variability of data, and the impact of different class distributions. This sub-metric will involve several parameters, including the performance of the model in few-shot scenarios, the complexity of the learning task, and the variability within the few-shot samples, more formally:

    \begin{LARGE}
    \begin{equation}
        FSLC = \frac{\mathcal{P}_{few\_shot}}{\mathcal{P}_{full}}  \times \frac{k}{C} \times \frac{1}{1 + \sigma}
    \end{equation}
    \end{LARGE}
    
     \textit{Key parameters:}
    \begin{itemize}
        \item $k$: Number of examples per class in the few-shot scenario (e.g., 1-shot, 5-shot).
        \item $C$: Number of classes or categories involved in the task.
        \item $\sigma$: Variability within the few-shot examples, measured as the standard deviation of features within the few-shot set.
        \item $\mathcal{P}_{few\_shot}$: Model performance in the few-shot scenario (e.g., accuracy, F1 score).
        \item $\mathcal{P}_{full}$: Model performance using a fully labeled dataset.
    \end{itemize}.

    A higher value suggests strong few-shot learning capabilities.


    \textbf{Data Noise Robustness (DNR):} Evaluates a model's ability to maintain its performance in the presence of various types and levels of noise in the dataset. Noise can include random errors, missing values, outliers, or label noise that corrupts the dataset and introduces inconsistencies. This sub-metric measures how resilient the model is when exposed to noisy data by comparing its performance on clean versus noisy datasets. A high DNR score indicates that the model is robust and able to handle data imperfections effectively, which is critical for real-world applications where data quality is often sub-optimal.



    \begin{LARGE}
    \begin{equation}
        DNR = \frac{\sum_{i=1}^n \sum_{j=1}^m w_{i,j} \times \big( \frac{\mathcal{P}_{\eta_i , \tau_j}}{\mathcal{P}}\big)}{\sum_{i=1}^n \sum_{j=1}^m w_{i,j}}
    \end{equation}
    \end{LARGE}

    where $\eta_i$ represents the level of noise, indicating how much noise (e.g., 10\%, 20\%, or 50\%) is applied to the data, $\tau_j$ indicates the type of noise, such as Gaussian noise, missing data, outliers, or label noise. $w_{i,j}$ is the weight assigned to each combination of noise level 
    $\eta_i$ and noise type $\tau_j$, reflecting the relative importance of each noise scenario.


    \textbf{Data Augmentation Sensitivity (DAS):} Measures the effectiveness of data augmentation techniques in enhancing model performance, reflecting the model's ability to leverage synthetic data effectively. It is calculated by comparing the performance improvement when augmentation techniques are applied versus when they are not, more formally:

    \begin{LARGE}
    \begin{equation}
        DAS = \left( 1 + \frac{\mathcal{P}_{augmented} - \mathcal{P}_{original}}{\left( \frac{\mathcal{P}_{original} + \mathcal{P}_{augmented}}{2} \right)} \right) / 2
    \end{equation}
    \end{LARGE}
    	
     Higher sensitivity indicates better use of augmented data to boost learning efficiency.



     \item \textbf{Resource Utilization Efficiency (RUE):} Measures how efficiently the model uses resources (CPU, memory) relative to its performance as dataset size scales up. It Compares the performance-to-resource ratio between small and large datasets, more formally:
    
    \begin{LARGE}
    \begin{equation}
        RUE = \frac{\mathcal{P}_{large} / \mathcal{RC}_{large}}{\mathcal{P}_{small} / \mathcal{RC}_{small}}
    \end{equation}
    \end{LARGE}
    
    where $\mathcal{P}_{large}$ and $\mathcal{P}_{small}$ refers to the performance value (e.g., accuracy, F1 score, etc.) of \textit{large} and \textit{small} datasets, respectively. Similarly, $\mathcal{RC}_{large}$ and $\mathcal{RC}_{small}$ determine the resource consumption values (e.g., CPU core hours for cup utilization) for large and small datasets, respectively.
    A value close to 1 indicates that resource usage scales well with performance.

    \item \textbf{Computational Scalability (CS):} Assesses how well the model handles increased computational demands as the dataset grows. 
    It evaluates the change in computational resource usage relative to the increase in dataset size.
    
    \begin{LARGE}
    \begin{equation}
        CS = \frac{ \mathcal{RC}_{large} - \mathcal{RC}_{small}}{\log{\left( \frac{|Dataset_{large}|}{|Dataset_{small}|} \right)}}
    \end{equation}
    \end{LARGE}


    Here, $|Dataset_{large}|$ refers to the size of the \textit{large} dataset, and $|Dataset_{small}|$ for the \textit{small} dataset, similarly.
    This formula helps identify if the model is becoming disproportionately resource-intensive as data size increases.

    \item \textbf{Feature Scalability (FS):} Measures how well the model performs as the number of features grows, reflecting adaptability to high-dimensional data. It Compares performance as the number of features increases, with an adjustment for feature growth, more formally:
    
    \begin{LARGE}
    \begin{equation}
        FS = \frac{\mathcal{P}_{highF}}{\mathcal{P}_{lowF}} \times \frac{1}{1 + \log{ \left( \Delta\mathcal{F} \right)}}
    \end{equation}
    \end{LARGE}

    where $\mathcal{P}_{highF}$ and $\mathcal{P}_{lowF}$ represent the performance values for the tables with a high number of features and a low number of features, respectively, $\Delta\mathcal{F}$ refers to the differences between high and low feature sets' size.
    This approach penalizes models that struggle with more complex feature spaces.

    \item \textbf{Training Time Efficiency (TTE):} Evaluates how training time scales relative to the performance gained as dataset size increases. It is assessed by comparing the increase in training time to the corresponding performance improvement, more formally:
    
    \begin{LARGE}
    \begin{equation}
        TTE = \frac{\mathcal{P}_{large} - \mathcal{P}_{small}}
        {\mathcal{T}_{large} - \mathcal{T}_{small}}
    \end{equation}
    \end{LARGE}

    Here, $\mathcal{T}_{large}$ and $ \mathcal{T}_{small}$ indicate the training time values for large and small datasets, respectively.
    A higher value indicates that additional training time is yielding significant performance gains.



     \textbf{Model Transparency Score (MTS):} Assesses how transparent the model structure is, reflecting how easily humans can understand the model’s architecture and the flow of information. It is scored based on the model complexity index ($\mathcal{C}$), such as the number of layers in neural networks or the depth of decision trees, adjusted for interpretability factors like modularity and simplicity, more formally:
    
    \begin{LARGE}
        \begin{equation}
            MTS = \frac{\mathcal{I}}{1 + \mathcal{C}}
        \end{equation}
    \end{LARGE}
    
    where

    \begin{LARGE}
        \begin{equation}
            \mathcal{C} = \frac{\mathcal{L}}{\mathcal{L}_{max}} + \frac{\log(\mathcal{P})}{\log(\mathcal{P}_t{max})} + \frac{\mathcal{N}}{\mathcal{N}_{max}} + \frac{\mathcal{A}}{\mathcal{A}_{max}}
        \end{equation}
    \end{LARGE}

in which:
\begin{itemize}

    \item \textit{$\mathcal{I}$:} The combined interpretability factor, is adjusted for transformer models by considering modularity, sparsity, and specific transformer interpretability techniques (e.g., attention visualization).

    \item \textit{Number of Layers ($\mathcal{L}$):} Reflects the depth of the architecture.
    
    \item \textit{Number of Parameters ($\mathcal{P}$):} Reflects the size and capacity of the model.
    
    \item \textit{Attention Heads ($\mathcal{A}$):} Specific to transformers, the number of attention heads contributes to both complexity and interpretability challenges.
    
    \item \textit{Non-linearities ($\mathcal{N}$):} Includes activation functions and complex pathways created by attention mechanisms.

    
\end{itemize}
    
    
\textbf{Local Interpretability (LI):} Measures how well the model can provide understandable explanations for individual predictions (e.g., through methods like SHAP values or LIME). It is evaluated by the accuracy of local explanation methods in representing the model’s behavior in specific instances, more formally:
    
    \begin{LARGE}
    \begin{equation}
        LI = \frac{\sum_{i=1}^{m} ACC_{explanation_j}}{m}
    \end{equation}
    \end{LARGE}
    
    This formula averages the accuracy of local explanations across multiple samples.



    \textbf{Predictive Parity Bias Score (PPBS):} Assesses whether the precision (positive predictive value) is consistent across groups, indicating if the model's positive predictions are equally reliable for all populations, more formally:
    
    \begin{LARGE}
    \begin{equation}
        PPBS = 1 - \frac{\sum_{i=1}^n \left| PPV_i - PPV_{avg} \right|}{n}
    \end{equation}
    \end{LARGE}
    
    where $PPV_i$ is the Positive Predictive Value (Precision) for group $i$, $PPV_{avg}$ is the average Positive Predictive Value across all groups, and $n$ is the number of groups. Higher values indicate less predictive bias across groups.

    \textbf{Bias Amplification Score (BAS):} Measures the extent to which the model amplifies existing biases present in the training data. This metric compares the bias in predictions with the bias inherent in the training data.
    
    \begin{LARGE}
    \begin{equation}
        BAS = 1 - \frac{ \sum_{i=1}^n \left| B_{predict_i} - B_{data_i} \right|}{n}
    \end{equation}
    \end{LARGE}
    
    where $B_{predict_i}$ is the bias level (e.g., the difference in mean outcomes) in predictions for group $i$, $B_{data_i}$ is the bias level in the training data for group $i$, and $n$ is the number of groups. Values near 1 suggest the model does not amplify training data biases significantly.





table

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        num & TFM Name & \multicolumn{10}{|c|}{Quality Metrics (Sub-metrics)} \\ \hline 
        %& Privacy Preservation & Data-Efficient Learning & Scalability & Interpretability &Fairness and Bias Mitigation\\
         \multirow{9}{2em}{1} & \multirow{9}{5.5em}{TransTab} & \multicolumn{5}{|c|}{Generalizability} & \multicolumn{5}{|c|}{Privacy Preservation} \\ \cline{3-7} \cline{8-12}
         & & IDT & CDT & SR & FAC & ZIA &DAR& MIR& DPC& DRAR& TPDHC\\ \cline{3-12} 
         &&1 & 1 & 1 & 1 & 1& 1 & 1 & 1 & 1 & 1\\ \cline{3-12}
         &&\multicolumn{5}{|c|}{Data-Efficient Learning} & \multicolumn{5}{|c|}{Scalability} \\ \cline{3-7} \cline{8-12}
         & & PRD& FLC& DNR &\multicolumn{2}{|c|}{DAS}& RUE& CS& FS& \multicolumn{2}{|c|}{TTE}\\ \cline{3-12} 
         &&1 & 1 & 1 & \multicolumn{2}{|c|}{1}& 1 & 1 & 1 & \multicolumn{2}{|c|}{1}\\ \cline{3-12}
         &&\multicolumn{5}{|c|}{Interpretability} & \multicolumn{5}{|c|}{Fairness and Bias Mitigation} \\ \cline{3-7} \cline{8-12}
         & & FIC& MTS& EC &\multicolumn{2}{|c|}{LI}& \multicolumn{3}{|c|}{PPBS}& BAS& IFS\\ \cline{3-12} 
         &&1 & 1 & 1 & \multicolumn{2}{|c|}{ 1}& \multicolumn{3}{|c|}{ 1} & 1 & 1\\ \hline
    \end{tabular}
    \caption{Tabular Foundation Models' Characteristics illustrated by the values of its corresponding sub-metrics}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|p{0.2cm}|p{0.8cm}|c|p{0.7cm}|c|p{0.6cm}|p{0.5cm}|c|c|c|c|c|c|c|c|}
    \hline
        \verb|#| & TFM & \multicolumn{13}{|c|}{Quality Sub-metrics} \\ \hline 
        \multirow{4}{5em}{1} & \multirow{4}{5em}{\rotatebox[origin=c]{90}{TransTab}} & IDT & CDT & SR & FAC & ZIA & DAR & MIR & DPC & DRAR & \multicolumn{2}{|c|}{TPDHC} & PRD & FLC \\ \cline{3-15} 
        && 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \multicolumn{2}{|c|}{1} & 1 & 1\\ \cline{3-15}
        && DNR & DAS & RUE & CS & FS & TTE & FIC & MTS & EC & LI & PPBS & BAS & IFS\\ \cline{3-15} 
        && 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\ \hline
        \multirow{4}{5em}{2} & \multirow{4}{5em}{\rotatebox[origin=c]{90}{TabNet}} & IDT & CDT & SR & FAC & ZIA & DAR & MIR & DPC & DRAR & \multicolumn{2}{|c|}{TPDHC} & PRD & FLC \\ \cline{3-15} 
        && 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \multicolumn{2}{|c|}{1} & 1 & 1\\ \cline{3-15}
        && DNR & DAS & RUE & CS & FS & TTE & FIC & MTS & EC & LI & PPBS & BAS & IFS\\ \cline{3-15} 
        && 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1\\ \hline
    \end{tabular}
    \caption{Tabular Foundation Models' Characteristics illustrated by the values of its corresponding sub-metrics}
    \label{tab:my_label}
\end{table}






    properties


    


\begin{table}[h!]
\centering
\small
\begin{tabular}{|p{3cm}|p{6cm}|p{6cm}|}
\hline
\textbf{Property (Abbrev.)} & \textbf{Brief Description} & \textbf{Effect on Sub-metrics}\\
\hline
Built-in Pre-Training Mechanism (BPTM) & The model includes a pre-training step on large, generic tabular data before fine-tuning. & Increases: IDT, CDT, FAC, PRD, FLC; Decreases: none. \\
\hline
Schema Adaptive Architecture (SAA) & The model can dynamically handle changes in the input schema without retraining. & Increases: SR, FAC; Decreases: none. \\
\hline
Advanced Feature Embeddings (AFE) & The model uses sophisticated embedding techniques for categorical and numerical features. & Increases: IDT, CDT, FAC; Decreases: DNR (if overly complex), DAS (if overly sensitive). \\
\hline
Zero-Shot Task Handling (ZSTH) & The model can infer on new tasks or domains without additional fine-tuning. & Increases: ZIA; Decreases: none. \\
\hline
On-Device Processing (ODP) & The model processes data locally without sending it to external servers. & Increases: DAR, MIR, DPC, DRAR, TPDHC; Decreases: none. \\
\hline
Differential Privacy Enforcement (DPE) & The model’s training procedure implements differential privacy mechanisms. & Increases: DPC, DAR, MIR, DRAR; Decreases: none. \\
\hline
Minimal External Data Transfer (MEDT) & The model avoids sending raw data to third parties, using only local computation or encrypted summaries. & Increases: TPDHC, DAR, MIR; Decreases: none. \\
\hline
Robustness to Missing Data (RMD) & The model can handle missing or incomplete features gracefully. & Increases: SR, DNR; Decreases: none. \\
\hline
Data Augmentation Compatibility (DAC) & The model maintains stable performance under various data augmentations. & Increases: DAS; Decreases: none. \\
\hline
Efficient Architecture Design (EAD) & The model’s architecture is optimized for memory and computation, reducing overhead. & Increases: RUE, CS, FS, TTE; Decreases: none. \\
\hline
Parallelization/Distributed Training Support (PDTS) & The model can be trained across multiple nodes/machines efficiently. & Increases: CS, TTE; Decreases: none. \\
\hline
Automated Feature Selection (AFS) & The model can automatically identify and focus on the most relevant features. & Increases: FAC, FS; Decreases: none. \\
\hline
Inherent Explainability Tools (IET) & The model offers built-in explanations of its predictions (e.g., feature importance scores). & Increases: FIC, MTS, EC, LI; Decreases: none. \\
\hline
Bias-Mitigation Techniques (BMT) & The model includes strategies (e.g., reweighting, adversarial training) to reduce bias. & Increases: PPBS, IFS; Decreases: BAS. \\
\hline
Intersectional Fairness Handling (IFH) & The model considers overlapping demographic groups to maintain fairness across them. & Increases: IFS, PPBS; Decreases: BAS. \\
\hline
Robust to Data Noise (RDN) & The model is resistant to performance degradation under noisy inputs. & Increases: DNR; Decreases: none. \\
\hline
Support for Few-Shot Adaptation (FSA) & The model can adapt to new tasks with only a few training examples. & Increases: FLC, PRD; Decreases: none. \\
\hline
Efficient Transfer Across Domains (ETAD) & The model can quickly adapt to new domains without extensive retraining. & Increases: CDT, IDT; Decreases: none. \\
\hline
Consistent Explanation Across Instances (CEAI) & The model provides stable and coherent explanations for different data samples. & Increases: EC, LI, MTS; Decreases: none. \\
\hline
Local Interpretability Mechanism (LIM) & The model supports interpretation of predictions at the instance level. & Increases: LI, EC; Decreases: none. \\
\hline
\end{tabular}
\caption{Properties of Tabular Foundation Models (TFMs) and Their Influence on Sub-metrics}
\label{tab:properties}
\end{table}


==> sections/TFMs.tex <==
\subsection{Extended List of Tabular Foundation Models}

\setlength{\tabcolsep}{3pt}

\begin{longtable}{|p{1.8cm}|c|c|c|c|c||c|c|c|c|c||c|c|c|}
\caption{Tabular Foundation Models' Characteristics (Extended Set, 45 models). Sub-metric scores are derived from documented design properties starting from a default value of 10, applying Table~\ref{tab:drawback_properties} uniformly to every model against its original publication (Section~\ref{sec:audit-note}); no model receives an exception to this rule. Models marked $^{\dagger}$ (P-Transformer, UniTTab, SPROUT, DTT, GPT4Table) could not be matched to a verifiable primary source under their listed name during this re-derivation and are placeholders pending correction; see Section~\ref{sec:audit-note} for detail.\label{tab:extended_models}}\\

\hline
\multirow{3}{5em}{TFM}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}IDT - CDT - SR - FAC - ZIA}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}DAR - MIR - DPC - DRAR - TPDHC}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}PRD - FLC} \\ \cline{2-14}
\rule{0pt}{10pt}
& \multicolumn{2}{|c|}{DNR - DAS}
& \multicolumn{4}{|c|}{RUE - CS - FS - TTE}
& \multicolumn{4}{|c|}{FIC - MTS - EC - LI}
& \multicolumn{3}{|c|}{PPBS - BAS - IFS} \\
\hline
\endfirsthead

\caption*{(continued)}\\
\hline
\multirow{3}{5em}{TFM}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}IDT - CDT - SR - FAC - ZIA}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}DAR - MIR - DPC - DRAR - TPDHC}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}PRD - FLC} \\ \cline{2-14}
\rule{0pt}{10pt}
& \multicolumn{2}{|c|}{DNR - DAS}
& \multicolumn{4}{|c|}{RUE - CS - FS - TTE}
& \multicolumn{4}{|c|}{FIC - MTS - EC - LI}
& \multicolumn{3}{|c|}{PPBS - BAS - IFS} \\
\hline
\endhead

\hline
\multicolumn{14}{r}{\textit{Continued on next page}} \\
\endfoot

\endlastfoot

% TransTab
\multirow{2}{4em}{TransTab}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{8 - 8 - 9 - 8}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabNet
\multirow{2}{4em}{TabNet}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% FT-Transformer
\multirow{2}{4em}{FT-Transformer}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 9}
& \multicolumn{4}{|c|}{10 - 10 - 8 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabTransformer
\multirow{2}{4em}{TabTransformer}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 9}
& \multicolumn{4}{|c|}{8 - 8 - 9 - 8}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% MediTab
\multirow{2}{4em}{MediTab}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 9 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabPFN
\multirow{2}{4em}{TabPFN}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabPFN v2
\multirow{2}{4em}{TabPFN~v2}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabPFN 2.5
\multirow{2}{4em}{TabPFN~2.5}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 10}
& \multicolumn{4}{|c|}{10 - 10 - 10 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabPFN 3
\multirow{2}{4em}{TabPFN~3}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 8 - 9}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% SAINT
\multirow{2}{4em}{SAINT}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% NODE
\multirow{2}{4em}{NODE}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabRet
\multirow{2}{4em}{TabRet}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{8 - 8 - 9 - 8}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% UniTabE
\multirow{2}{4em}{UniTabE}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% CARTE
\multirow{2}{4em}{CARTE}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% GReaT
\multirow{2}{4em}{GReaT}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabuLa
\multirow{2}{4em}{TabuLa}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{9 - 9 - 8 - 9}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% XTab
\multirow{2}{4em}{XTab}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 9}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabDPT
\multirow{2}{4em}{TabDPT}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{10 - 10 - 9 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabICL
\multirow{2}{4em}{TabICL}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 10}
& \multicolumn{4}{|c|}{10 - 10 - 10 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% VIME
\multirow{2}{4em}{VIME}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 10}
& \multicolumn{4}{|c|}{10 - 10 - 9 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabCaps
\multirow{2}{4em}{TabCaps}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 8 - 9 - 9}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{10 - 10 - 9 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabLLM
\multirow{2}{4em}{TabLLM}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% Table2Vec
\multirow{2}{4em}{Table2Vec}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{10 - 10 - 9 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% P-Transformer
\multirow{2}{4em}{P-Transformer $^{\dagger}$}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% FATA-Trans
\multirow{2}{4em}{FATA-Trans}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{10 - 10 - 9 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% UniTTab
\multirow{2}{4em}{UniTTab $^{\dagger}$}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 8 - 9 - 9}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabGPT
\multirow{2}{4em}{TabGPT}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 8 - 9 - 9}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TURL
\multirow{2}{4em}{TURL}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabBERT
\multirow{2}{4em}{TabBERT}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TUTA
\multirow{2}{4em}{TUTA}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TABBIE
\multirow{2}{4em}{TABBIE}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{8 - 8 - 8 - 8}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TAPEX
\multirow{2}{4em}{TAPEX}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TaBERT
\multirow{2}{4em}{TaBERT}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TAPAS
\multirow{2}{4em}{TAPAS}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TABLET
\multirow{2}{4em}{TABLET}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{10 - 10 - 8 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% HeLM
\multirow{2}{4em}{HeLM}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TAPTAP
\multirow{2}{4em}{TAPTAP}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{10 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabText
\multirow{2}{4em}{TabText}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{9 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% TabFM
\multirow{2}{4em}{TabFM}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{8 - 8 - 8 - 8}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% SPROUT
\multirow{2}{4em}{SPROUT $^{\dagger}$}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 8 - 9 - 9}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% REaLTabFormer
\multirow{2}{4em}{REaLTabFormer}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 10 - 10 - 10}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 10}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% UniPredict
\multirow{2}{4em}{UniPredict}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 9 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{10 - 10 - 8 - 10}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% DTT
\multirow{2}{4em}{DTT $^{\dagger}$}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9 - 8 - 9 - 9}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

% GPT4Table
\multirow{2}{4em}{GPT4Table $^{\dagger}$}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}10 - 10 - 8 - 10 - 10}
& \multicolumn{5}{|c|}{\cellcolor[HTML]{D3D3D3}8 - 8 - 8 - 8 - 8}
& \multicolumn{3}{|c|}{\cellcolor[HTML]{D3D3D3}9 - 9}\\ \cline{2-14}
& \multicolumn{2}{|c|}{8 - 9}
& \multicolumn{4}{|c|}{7 - 7 - 8 - 7}
& \multicolumn{4}{|c|}{9 - 9 - 9 - 9}
& \multicolumn{3}{|c|}{9 - 9 - 9}\\ \hline

\end{longtable}

